DN-DETR: Accelerate DETR Training by Introducing Query DeNoising

We present in this paper a novel denoising training method to speedup DETR (DEtection TRansformer) training and offer a deepened understanding of the slow convergence issue of DETR-like methods. We show that the slow convergence results from the instability of bipartite graph matching which causes inconsistent optimization goals in early training stages. To address this issue, except for the Hungarian loss, our method additionally feeds ground-truth bounding boxes with noises into Transformer decoder and trains the model to reconstruct the original boxes, which effectively reduces the bipartite graph matching difficulty and leads to a faster convergence. Our method is universal and can be easily plugged into any DETR-like methods by adding dozens of lines of code to achieve a remarkable improvement. As a result, our DN-DETR results in a remarkable improvement ($+1.9$AP) under the same setting and achieves the best result (AP $43.4$ and $48.6$ with $12$ and $50$ epochs of training respectively) among DETR-like methods with ResNet-$50$ backbone. Compared with the baseline under the same setting, DN-DETR achieves comparable performance with $50\%$ training epochs. Code is available at \url{https://github.com/FengLi-ust/DN-DETR}.

==> cvpr2022/SUP.tex <==
\section{Appendix}
\subsection{Other tasks and future work}
\subsubsection{Other Tasks}
% We demonstrate some potential abilities of our method and some attempts we have made.
 In addition to regular detection, our design of queries as anchor box + label makes the detection model capable of handling other tasks. For example, known objects detection and known labels detection. Note that results shown in this section are just a preliminary exploration and not based on our well trained model with best hyper-parameters.

\noindent\textbf{Known Objects Detection: } Assume we know a part of the objects in an image and want to predict the remaining objects. We want the known objects to help predict the unknown objects through co-occurrence relations. We did some preliminary exploration. We randomly divide the $80$ classes of MSCOCO2017 into $2$ parts including known classes and unknown classes. We put objects of known classes in denoising part and want the matching part to predict the objects of the unknown classes. We do not use attention mask so that the matching part can get useful information from the denoising part. Our experimental results is shown in Table \ref{tab:extra_label}. Compared with the evaluation without known boxes, the known objects evaluation improves the performance, which indicates that co-occurrence helps the prediction of unknown boxes. Moreover, our DN-DETR trained with known objects exceeds DAB-DETR only trained on unknown classes when evaluating without known objects. This means the denoising of extra boxes from extra (known) classes also helps the performance on the unknown objects.
\input{cvpr2022/tables/conditional_prediction}

\noindent\textbf{Known Labels Detection: } For each image, we assume we know all the class labels in the image without box information. Since our model has interpreted the query embedding into class label embedding, we can seamlessly utilize these known labels to detect the boxes of each class label. For each class $c$ in the image, we concatenate its label embedding with the indicator $1$ which denotes known label. We feed the concatenated vector into the decoder and let the decoder output all boxes of class $c$. To compare with methods without known boxes. We concatenate outputs of all classes and evaluate the result as shown in Table \ref{tab:known_label}.
Within $10$ epochs of finetuning on pretrained DN-DETR, the known label detection performance is improved to $46.6$.
\input{cvpr2022/tables/known_label}
\subsubsection{future work}
There are two potential future works to be mentioned here. One is zeroshot detection and the other is progressive inference.\\
\textbf{Zeroshot Detection :} Since we have decoupled decoder queries as anchor boxes and class labels, pretrained class label embeddings can be fed into the class label part of the queries. To enable zeroshot detection, one can take $80$ classes of MSCOCO as phrases and collect phrase embeddings from a pretrained language model as the class label embedding. With the pretrained label embedding, it is possible to train a given class detector which takes a class label embedding as input and detect objects of the given classes. In inference time, class label embeddings from unseen classes can be fed into the decoder to achieve zeroshot detection.

\noindent\textbf{Progressive inference}
Based on the known objects detection, a progressive inference method can be designed. For example, we can train a DN-DETR capable of doing known objects detection. In inference time, we let the detector predict objects and then, we can choose the objects with highest score and treat them as known objects to do known objects detection. For each step of prediction, we choose objects with highest score and add them to the known boxes set. After repeating for many times, we get the final prediction.
\newpage




==> cvpr2022/tables/main_results.tex <==
\begin{table*}[t]
    \centering
    %     \footnotesize
    %         \renewcommand{\arraystretch}{1.6}
    % \resizebox{\columnwidth}{!}{%
    \begin{tabular}{lccccccccccc}
        \toprule
        Model & MultiScale & \#epochs & AP & AP$_{50}$ & AP$_{75}$ & AP$_{S}$ & AP$_{M}$ & AP$_{L}$ & GFLOPs & Params \\
        \midrule
        \midrule
        % Faster R$50$-C4 1x& & $12$ & $35.7$ & $--$ & $--$ & $--$ & $--$ & $--$ & $--$M\\
        Faster R$50$-DC5 1x& & $12$ & $37.3$ & $--$ & $--$ & $--$ & $--$ & $--$ & $--$M\\
        Faster R$50$-FPN 1x& & $12$ & $37.9$ & $--$ & $--$ & $--$ & $--$ & $--$ & $--$M\\
        DAB-DETR-DC5-R$50^*$& & $12$ & $--$ & $--$ & $--$ & $--$ & $--$ & $--$ & $--$M\\
        Dynamic DETR -R$50$ 1x& & $12$ & $40.2$ & $--$ & $--$ & $--$ & $--$ & $--$ & $--$M\\
        % R$50$-C4 3x& & $36$ & $38.4$ & $--$ & $--$ & $--$ & $--$ & $--$ & $--$M\\
        % R$50$-DC5 3x& & $36$ & $39.0$ & $--$ & $--$ & $--$ & $--$ & $--$ & $--$M\\
        % DN-DETR-R$50$& & $36$ & $42.2$ & $62.6$ & $44.8$ & $21.4$ & $45.8$ & $61.7$ & $44$M \\
        DN-DETR-DC5-R$50$& & $12$ & $\textbf{40.7}$ & $--$ & $--$ & $--$ & $--$ & $--$ & $--$M\\
        DN-DETR-DC5-R$50^*$& & $12$ & $\textbf{41.6}$ & $--$ & $--$ & $--$ & $--$ & $--$ & $--$M\\
        Faster R$101$ FPN 3x& & $36$ & ${42.0}$ & $--$ & $--$ & $--$ & $--$ & $--$ & $--$M\\
        DN-DETR-DC5-R$101^*$& & $12$ & $\textbf{42.8}$ & $--$ & $--$ & $--$ & $--$ & $--$ & $--$M\\
        \hline
        \hline
        DETR-R$50$                & & $500$ & $42.0$ & $62.4$ & $44.2$ & $20.5$ & $45.8$ & $61.1$ & $86$ & $41$M \\
        Faster RCNN-FPN-R$50$   & & $108$ & $42.0$  & $62.1$ & $45.5$ & $26.6$ & $45.5$ & $53.4$ & $180$ & $42$M \\
        Anchor DETR-R$50$         & & $50$ & $42.1$ & $63.1$ &  $44.9$ &  $22.3$ &  $46.2$  & $60.0$ & $-$ & $39$M \\
        Conditional DETR-R$50$    & & $50$ & $40.9$ & $61.8$ & $43.3$ & $20.8$ & $44.6$ & $59.2$ & $90$ & $44$M \\
        DAB-DETR-R$50$    & & $50$ & $42.2$ & $63.1$ & $44.7$ & $21.5$ & $45.7$ & $60.3$ & $94$ & $44$M \\
        % DN-DETR-R$50$    & & $\textbf{35}$ & $42.2$ & $62.6$ & $44.8$ & $21.4$ & $45.8$ & $61.7$ & $--$ & $44$M \\
        % DN-DETR-R$50$     & & $50$ & $\textbf{43.4}$ & $63.8$ & $45.9$ & $22.9$ & $46.9$ & $62.9$ & $--$ & $44$M \\
        DN-DETR-R$50$& & $50$ & $\textbf{44.1}$ & $64.4$ & $46.7$ & $22.9$ & $48.0$ & $63.4$ & $--$ & $44$M \\
        % DAB-DETR-R$50^{*}$    & & $50$ & {${42.6}$} & $63.2$ & $45.6$ & $21.8$ & $46.2$ & $61.1$ & $100$ & $44$M \\
        % DN-DETR-R$50^*$    & & $50$ & $--$ & $--$ & $--$ & $--$ & $--$ & $--$ & $--$ & $--$M \\
        % DAB-DETR-R$50^{-}$    & & $50$ & $42.2$ & $63.1$ & $44.7$ & $21.5$ & $45.7$ & $60.3$ & $94$ & $44$M \\
        % DAB-DETR-R$50^{*}$    & & $50$ & $42.5$ & $63.2$ & $45.1$ & $23.7$ & $46.5$ & $61.4$ & $100$ & $44$M \\
        % DAB-DETR-R$50$    & & $50$ & {$\textbf{{42.6}}$} & $63.2$ & $45.6$ & $21.8$ & $46.2$ & $61.1$ & $100$ & $44$M \\
        \hline
        DETR-R$101$                & & $500$ & $43.5$ & $63.8$ & $46.4$ & $21.9$ & $48.0$ & $61.8$ & $152$ & $60$M \\
        Faster RCNN-FPN-R$101$  & & $108$ & $44.0$ & $63.9$ & $47.8$ & $27.2$ & $48.1$ & $56.0$ & $246$ & $60$M \\
        Anchor DETR-R$101$         & & $50$ & $43.5$ &  $64.3$ &  $46.6$ &  $23.2$  & $47.7$  & $61.4$ & $-$ & $58$M \\
        Conditional DETR-R$101$   & & $50$ & $42.8$ &  $63.7$ &  $46.0$ &  $21.7$ &  $46.6$ &  $60.9$  & $156$ & $63$M\\
        DAB-DETR-R$101$    & & $50$ & {${43.5}$} & $63.9$ & $46.6$ & $23.6$ & $47.3$ & $61.5$ & $174$ & $63$M \\
        DN-DETR-R$101$    & & $50$ & {$\textbf{45.0}$} & $65.2$ & $48.3$ & $25.2$ & $49.2$ & $63.9$ & $--$ & $63$M \\
        % DAB-DETR-R$101^{*}$    & & $50$ & {$\textbf{44.1}$} & $64.7$ & $47.2$ & $24.1$ & $48.2$ & $62.9$ & $179$ & $63$M \\
        % DAB-DETR-R$101^{-}$    & & $50$ & {${43.5}$} & $63.9$ & $46.6$ & $23.6$ & $47.3$ & $61.5$ & $174$ & $63$M \\
        % DAB-DETR-R$101^{*}$    & & $50$ & {${44.0}$} & $64.6$ & $47.1$ & $24.6$ & $47.9$ & $62.6$ & $179$ & $63$M \\
        % DAB-DETR-R$101$    & & $50$ & {$\textbf{44.1}$} & $64.7$ & $47.2$ & $24.1$ & $48.2$ & $62.9$ & $179$ & $63$M \\
        \hline
        \hline
        DETR-DC5-R$50$            & & $500$ & $43.3$ & $63.1$ & $45.9$ & $22.5$ & $47.3$ & $61.1$ & $187$ & $41$M \\
        Deformable DETR-R$50$   & \checkmark & $50$ & $43.8$ & $62.6$ & $47.7$ & $26.4$ & $47.1$ & $58.0$  & $173$ & $40$M \\ 
        SMCA-R$50$                & \checkmark & $50$ &  $43.7$ &  $63.6$ &  $47.2$ &  $24.2$ &  $47.0$ &  $60.4$ & $152$ & $40$M \\
        TSP-RCNN-R$50$          & \checkmark & $96$ & $45.0$ & $64.5$ & $49.6$ & $29.7$ & $47.7$ & $58.0$ & $188$ & $-$ \\
        Anchor DETR-DC5-R$50$         & & $50$ & $44.2$ & $64.7$ & $47.5$ & $24.7$ & $48.2$ & $60.6$ & $151$ & $39$M \\
        Conditional DETR-DC5-R$50$  & & $50$  &  $43.8$ & $64.4$ &  $46.7$ &  $24.0$ & $47.6$ &  $60.7$ & $195$ & $44$M \\
        DAB-DETR-DC5-R$50$    & & $50$ & {${44.5}$} & $65.1$ & $47.7$ & $25.3$ & $48.2$ & $62.3$ & $202$ & $44$M \\
        % DN-DETR-DC5-R$50$    & & $50$ & $\textbf{45.6}$ & $65.6$ & $48.6$ & $25.2$ & $49.4$ & $63.9$ & $--$ & $--$M \\
        DN-DETR-DC5-R$50$    & & $50$ & $\textbf{46.2}$ & $65.6$ & $48.6$ & $25.2$ & $49.4$ & $63.9$ & $--$ & $--$M \\
        DAB-DETR-DC5-R$50^{*}$    & & $50$ & {$45.7$} & $66.2$ & $49.0$ & $26.1$ & $49.4$ & $63.1$ & $216$ & $44$M \\
        DN-DETR-DC5-R$50^*$    & & $50$ & $\textbf{46.8}$ & $66.7$ & $49.8$ & $27.1$ & $50.1$ & $64.7$ & $--$ & $--$M \\
        % DAB-DETR-DC5-R$50^{-}$    & & $50$ & {${44.5}$} & $65.1$ & $47.7$ & $25.3$ & $48.2$ & $62.3$ & $202$ & $44$M \\
        % DAB-DETR-DC5-R$50^{*}$    & & $50$ & {${45.2}$} & $65.5$ & $48.5$ & $25.7$ & $48.8$ & $62.8$ & $216$ & $44$M \\
        % DAB-DETR-DC5-R$50$    & & $50$ & {$\textbf{45.7}$} & $66.2$ & $49.0$ & $26.1$ & $49.4$ & $63.1$ & $216$ & $44$M \\
        \hline 
        
        \hline 
        DETR-DC5-R$101$           & & $500$ & $44.9$ & $64.7$ & $47.7$ & $23.7$ & $49.5$ & $62.3$ & $253$ & $60$M \\
        TSP-RCNN-R$101$         & \checkmark & $96$ & $46.5$ & $66.0$ & $51.2$ & $29.9$ & $49.7$ & $59.2$ & $254$ & $-$\\
        SMCA-R$101$                & \checkmark & $50$ &  $44.4$ &  $65.2$ &  $48.0$ &  $24.3$ &  $48.5$ &  $61.0$ & $218$ & $50$M \\
        Anchor DETR-R$101$         & & $50$ & $45.1$ & $65.7$ & $48.8$ & $25.8$ & $49.4$ & $61.6$ & $-$ & $58$M \\
        Conditional DETR-DC5-R$101$  & & $50$  &   $45.0$ & $65.5$ & $48.4$ & $26.1$ & $48.9$ & $62.8$ & $262$ & $63$M \\
        DAB-DETR-DC5-R$101$    & & $50$ & {${45.8}$} & $65.9$ & $49.3$ & $27.0$ & $49.8$ & $63.8$ & $282$ & $63$M \\
        DN-DETR-DC5-R$101$    & & $50$ & $\textbf{46.5}$ & $66.6$ & $50.0$ & $27.0$ & $50.8$ & $64.8$ & $--$ & $--$M \\
        DAB-DETR-DC5-R$101^{*}$    & & $50$ & {$46.6$} & $67.0$ & $50.2$ & $28.1$ & $50.5$ & $64.1$ & $296$ & $63$M \\
        DN-DETR-DC5-R$101^*$    & & $50$ & $\textbf{47.8}$ & $67.7$ & $51.5$ & $27.4$ & $52.1$ & $66.2$ & $--$ & $--$M \\
        % DAB-DETR-DC5-R$101^{-}$    & & $50$ & {${45.8}$} & $65.9$ & $49.3$ & $27.0$ & $49.8$ & $63.8$ & $282$ & $63$M \\
        % DAB-DETR-DC5-R$101^{*}$    & & $50$ & {${46.3}$} & $66.9$ & $49.8$ & $27.0$ & $50.7$ & $64.1$ & $296$ & $63$M \\
        % DAB-DETR-DC5-R$101$    & & $50$ & {$\textbf{46.6}$} & $67.0$ & $50.2$ & $28.1$ & $50.5$ & $64.1$ & $296$ & $63$M \\
        \bottomrule
    \end{tabular}
    
    \centering
    \caption{Results for our Denoise-DETR and other detection models. 
    All DETR-like models except DETR use $300$ queries, while DETR uses $100$.
    The models with superscript $^{*}$ use $3$ pattern embeddings as in Anchor DETR~\cite{wang2021anchor}.
    }
    \label{tab:main_results}
    % \vspace{-.3cm}
\end{table*}
